Theories and Experiments for Testable Baryogenesis Mechanisms: A Snowmass White Paper

The baryon asymmetry of the Universe is one of the central motivations to expect physics beyond the Standard Model. In this Snowmass white paper, we review the challenges and opportunities in testing some of the central paradigms that predict physics at scales low enough to expect new experimental data in the next decade. Focusing on theoretical ideas and some of their experimental implications, in particular, we discuss neutron-antineutron transformations, flavor observables, next generation colliders, future neutron facilities, gravitational waves, searches for permanent electric dipole moments, $0\nu \beta \beta $ decay and some future large underground experiments as methods to test post-sphaleron baryogenesis, electroweak baryogenesis, mesogenesis and low scale leptogenesis. Finally, we comment on the cases where high scale physics can be probed through some of these same mechanisms.

==> subfiles/temp.tex <==




The experimental observation of neutrino ($\nu$) masses indicates the existence of new elementary particles beyond the SM.
At tree level it can be conveniently
explained by tree-level physics through the \emph{see-saw} 
mechanisms of
type-I\citep{Minkowski:1977sc,Mohapatra:1979ia,Glashow:1979nm,GellMann:1980vs,Yanagida:1980xy,Schechter:1980gr} 
  type-II\citep{Schechter:1980gr,Magg:1980ut,Cheng:1980qt,Lazarides:1980nt,Mohapatra:1980yp} and type-III\citep{Foot:1988aq}. In addition, many radiative models exist\citep{Cai:2017jrq}, including many that can connect to the Dark Matter problem\citep{Restrepo:2013aga}. 
%\citep{Minkowski:1977sc,Gell-Mann:1979vob,Yanagida:1980xy}. 
Leptogenesis\citep{Fukugita:1986hr} is an attractive scenario in which the matter-antimatter asymmetry of the observable universe\citep{Canetti:2012zc} is related to the properties of $\nu$s, allowing to constrain the parameter space with data from $\nu$ oscillation experients.
While leptogenesis was first proposed in the type I seesaw, it can also be realised with scalar\citep{Ma:1998dx} or fermionic\citep{Hambye:2003rt,Albright:2003xb} triplets or combinations thereof\citep{Antusch:2004xy}, cf.\citep{Hambye:2012fh} for a review, but the type I incarnation remains to be the most studied one on which we focus here.


\section{Low scale seesaw and leptogenesis} 


%In the case of its \emph{type I} realisation, 
%the introduction of additional \emph{heavy neutral leptons} (HNLs) opens the \emph{leptogenesis} pathway\citep{Fukugita:1986hr} for the generation of the BAU. 
A generic prediction of the type I seesaw is the existence of Heavy Neutral Leptons (HNLs) with Majorana masses near the seesaw scale.
The Yukawa couplings of the HNLs to the lepton doublets introduce
new sources of CP violation and the SM sphalerons violate baryon+lepton
number. If HNLs are out of thermal equilibrium at any temperature higher
than that of sphaleron decoupling --- 130 GeV approximately for the 
SM\citep{DOnofrio:2014rug} --- then all of Sakharov's conditions for 
successful baryogenesis are satisfied. 
Traditionally it was believed that leptogenesis requires very large Majorana masses for the HNLs\citep{Davidson:2002qv}.\footnote{See\citep{Buchmuller:2005eh,Davidson:2008bu,Bodeker:2020ghk,DiBari:2021fhs} for reviews on high scale leptogenesis and\citep{Dev:2017trv,Drewes:2017zyw,Dev:2017wwc,Biondini:2017rpb,Chun:2017spz,Hagedorn:2017wjy} for reviews on individual aspects of both, high and low scale leptogenesis.} 
In such high scale scenarios the HNLs are inaccessible to direct searches, though the mechanism can in principle be falsified\citep{Deppisch:2013jxa} by combining collider data with searches for neutrinoless double $\beta$-decay ($0\nu\beta\beta$)\citep{Deppisch:2015yqa}, cf.~Sec.~\ref{sec:HighScaleLepto}.
However, it is now established that HNLs with masses below the TeV scale can generate the observed BAU during both their production\citep{Akhmedov:1998qx,Asaka:2005pn} and/or freeze-out and decay\citep{Pilaftsis:2003gt,Pilaftsis:2005rv, Dev:2014pfm}. These mechanisms can be embedded in theoretically well-motivated low scale seesaw scenarios\citep{Agrawal:2021dbo}  and open up the possibility to search for the HNLs at colliders\citep{Atre:2009rg,Deppisch:2015qwa,Cai:2017mow,Agrawal:2021dbo} and probe the origin of matter\citep{Chun:2017spz}. 
%In this contribution we concentrate on low-scale scenarios, whereby the mass scale of the HNLs is not significantly higher than the EW scale.
%We refer to\citep{Buchmuller:2005eh,Davidson:2008bu,Bodeker:2020ghk,DiBari:2021fhs} for reviews of \emph{thermal leptogenesis} with very massive HNLs ($M>10^6$ GeV) and $\mathcal{O}(1)$ Yukawas.
%In order to have successful leptogenesis at masses much below these, as in our case, one needs that the masses of the HNLs --- two or more --- be sufficiently degenerate.

\subsection{Low scale leptogenesis mechanisms}

%What drives the HNL out of equilibrium in low-scale leptogenesis?
%It turns out that they 
The mechanisms driving low scale leptogenesis can be classified by the dominant cause of the deviation from equilibrium, namely the \emph{freeze-out} and \emph{freeze-in} mechanisms. 
In the former case, HNLs attain first thermal equilibrium early
on, to then fall out of it --- freeze out --- while sphalerons are still active.
They will then decay out of equilibrium, with the CP violation
of the Yukawas compounded by the mass degeneracy to give rise to
\emph{resonant leptogenesis}\citep{Liu:1993tg,Flanz:1994yx,Flanz:1996fb,Covi:1996wh,Covi:1996fm,Pilaftsis:1997jf,Buchmuller:1997yu,Pilaftsis:2003gt}. 
In the latter case, Yukawas are small enough that the HNLs cannot manage
to equilibrate before sphaleron freeze-out.
%CP violation is then ensuredby  \emph{oscillations}\citep{Akhmedov:1998qx,Asaka:2005pn} between their flavor states --- two at least. \textbf{Marco: oscillations happen i both scenarios}
It was long assumed that the freeze-out mechanism requires Majorana masses above the electroweak scale and the freeze-in mechanism only works with Majorana masses below the electroweak scale.
However, it has been recently pointed out\citep{Klaric:2020phc,Klaric:2021cpi}
that both mechanism in general coexist, and the assumption that one of them dominates only holds for $M \gg 1$ TeV\citep{Klaric:2020phc} or $M< 2$ GeV\citep{Drewes:2021nqr}. 
%this classification puts scenarios on a \emph{continuous spectrum},rather than in two discrete bins  which can then be understood as limiting cases.
%Their parameter spaces are overlapping,
%though, as one would expect, freeze in dominates at small, $M\lesssim\mathcal{O}$(GeV)
%masses, whereas freeze-out switches off at $M<2$ GeV. 

Low scale leptogenesis is technically more complicated than most high scale scenarios, due to thermal corrections to quasiparticle properties and reaction rates, the interplay between coherent oscillations and decoherent scatterings and a full flavour dependence. 
From the theoretical standpoint, computations of baryon asymmetry
production rely on techniques ranging from simple semi-classical Boltzmann
equations to more sophisticated approaches, such as the closed
time path (CTP) formalism or the operatorial approach based 
on scale separations, have been developed. We refer to these recent reviews\citep{Garbrecht:2018mrp,Biondini:2017rpb} for an
in-depth analysis of computational techniques. 
These have been used for both, precision calculations\citep{Ghiglieri:2018wbs,Ghiglieri:2020ulj}
as well as explorations of the viable parameters space \citep{Canetti:2010aw,Canetti:2012vf,Canetti:2012kh,Dev:2014oar, Hernandez:2015wna,Shuve:2014zua,Drewes:2016gmt,Hernandez:2016kel,Drewes:2016jae,Eijima:2018qke,Boiarska:2019jcw,Drewes:2021nqr,Klaric:2021cpi}.
The allowed parameter space overlaps with the sensitivity of many direct search experiments, see figure \ref{HNLsummary}.

\subsection{Testability and complementarity}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.415\textwidth]{figures/v51NHIH.pdf}\includegraphics[width=0.45\textwidth]{figures/snowmassDUNENOIO.pdf}
\caption{\label{fig:triangle}
Allowed range for the relative magnitude of the HNL mixings with indicifual SM flavours in the minimal type I seesaw model\citep{Verhaaren:2022ify}.
%, plot taken from \color{red}[Snowmass HNL WP, courtesty Juraj Klaric]\color{black}
 \textit{Left panel}: The range of normalized flavour mixings consistent with the current $\nu$ oscillation data 
 %in the $n=2$ case 
 (see e.g.\citep{Drewes:2016jae,Caputo:2017pit,Drewes:2018gkc}). The different contours correspond to the allowed $\Delta \chi^2$ range from\citep{Esteban:2020cvm} for the case of normal (red) and inverted (blue) light $\nu$ mass ordering.
\textit{Right panel}: The projected $90\%$ CL for the mixing ratios after 14 years of $\nu$ oscillation measurements at DUNE\citep{DUNE:2020jqi}.
For this projection we assume maximal CP violation $\delta=-\pi/2$ and two benchmark values of the PMNS angle $\theta_{23}$, used in the DUNE TDR\citep{DUNE:2020ypp}, indicated in the legend.
%fixing the known oscillation parameters to their best fit values\citep{Esteban:2020cvm} and varying the CP phases from $\left[0,2\pi\right]$ for NH (red) and IH (blue) in the minimal seesaw model.
}
\end{center}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=0.49\textwidth]{figures/HNLosc2.pdf}
\includegraphics[width=0.49\textwidth]{figures/MassSplittingLeptogenesis.pdf}
\caption{\label{leptogenesisn2}
Left: Idealised picture of the ratio of $L$-violating (LNV) and $L$-conserving (LNC) heavy $\nu$ decays as a function of position. The ratio oscillates due to coherent $N_i$ flavour oscillations\citep{Antusch:2017ebe}.
Right: Range of physical heave $\nu$ mass splitting $\Delta M_{\rm phys}$ and mixing $U^2=\sum_iU_i^2$ for which leptogenesis is feasible for $\bar{M}=30$ GeV (blue region), compared to the contribution $\Delta M_{\theta\theta}$ to $\Delta M_{\rm phys}$ from the Higgs mechanism\citep{Antusch:2017pkq}.
}
\end{figure*}

\begin{figure}[t!]
 \begin{center}
% \includegraphics[width=0.45\columnwidth]{figures/ship_plot} 
  \includegraphics[width=0.65\columnwidth]{figures/mbbIH.pdf} 
\caption{\label{fig:masterplot} %\emph{Left panel:} 
%Posterior probabilities in the %$|m_{\beta\beta}|$ vs baryon asymmetry $Y_B$ %plane 
%in the type I seesaw model with two HNL %flavours.
%after a measurement at SHiP (red), assuming
%$0.1\%, 1\%$ uncertainty on the measurement of the HNL masses and mixing respectively, and the an measurement of $\delta$ by T2HK or 
%DUNE (blue). See\citep{Hernandez:2016kel} for further details.
%\color{red}
%need to ask Jacobo for permission
\color{black}
%\emph{Right panel:}
Expected rate for $0\nu\beta\beta$ in the minimal type I seesaw with two right-handed $\nu$s (or the $\nu$MSM) in the allowed region from Fig.~\ref{fig:triangle} for inverted light $\nu$ mass ordering. A deviation from this prediction would be sensitive to the heavy $\nu$ mass splitting and the  phases in the sterile sector\citep{Asaka:2016zib}, an important ingredient to test leptogenesis\citep{Drewes:2016lqo,Hernandez:2016kel,Asaka:2016zib}. See Figure 11 in\citep{Hernandez:2016kel} also for posterior probabilities in the $|m_{\beta\beta}|$ vs baryon asymmetry $Y_B$ plane 
in the type I seesaw model with two HNL flavours.
}
\end{center}
\end{figure}


%\color{red}
%I would suggest to put figures 4.5 - 4.7 close to the paragraphs where they appear as they are now appearing in the wrong section.\\
\color{black}
If HNLs are discovered in any direct search, a pressing question will be whether these particles are indeed responsible for the origin of $\nu$ masses and the BAU. For this purpose one can take advantage that the parameter space is constrained by a wide range of indirect observables\citep{Drewes:2013gca,Antusch:2014woa,Gorbunov:2014ypa,Drewes:2015iva, deGouvea:2015euy,Fernandez-Martinez:2016lgt,Drewes:2016jae,Chrzaszcz:2019inj, Bolton:2019pcu}. Some points include:
\begin{itemize}
\item The requirement to reproduce the observed pattern of light $\nu$ mixing imposes testable constraints on the relative size of the HNL couplings to individual SM flavors\citep{Hernandez:2016kel,Drewes:2016jae,Drewes:2018gkc,Chrzaszcz:2019inj}. These will improve in the future with DUNE, see  Fig.~\ref{fig:triangle}.
\item A confirmation of the Majorana nature of the HNLs can be achieved by observing lepton number violation (LNV) in their decays. The smallness of the light $\nu$ masses enforces an generalised $B-L$ symmetry on the viable parameter space of low scale seesaw scenarios\citep{Shaposhnikov:2006nn,Kersten:2007vk}, implying that HNLs with collider-accessible couplings with the SM must be organised in pseudo-Dirac pairs\citep{Moffat:2017feq}. The resulting (approximate) $B-L$ conservation in principle parametrically suppresses all LNV processes at colliders\citep{Kersten:2007vk,Ibarra:2010xw}, but can be overcome if the HNL lifetime exceeds their oscillation length\citep{Anamiati:2016uxp} through oscillations between the two HNLs\citep{Boyanovsky:2014una,Antusch:2020pnn} with different lepton number. 
Even if the final state cannot be fully reconstructed, the angular distribution of decay products can be\citep{Kayser:1982br,Balantekin:2018ukw,Tastet:2019nqj,Blondel:2021mss,deGouvea:2021rpa}; similarly, decays into different flavors\citep{Dib:2016wge} can be sensitive to the LNV.
These effects have been studied for the LHC\citep{Dib:2017iva,Das:2017hmg}, ILC\citep{Hernandez:2018cgc}, NA62\citep{Abada:2019bac} and SHiP\citep{Tastet:2019nqj}. Generally one can expect LNV to observable in searches for long-lived HNLs, while it is suppressed in prompt decays\citep{Drewes:2019byd}; see Fig.~\ref{HNLsummary}.
\item Measuring the HNL flavour mixing pattern can permit indirect constraints on the Majorana phase in the $\nu$ mixing matrix\citep{Drewes:2016jae,Caputo:2016ojx}, while oscillations can give access to other CPV phases in the HNL sector\citep{Cvetic:2015naa,Cvetic:2015ura}.
The phases in the sterile sector can also be accessed within the viable leptogenesis parameter space by combining measurements of the HNL couplings to individual SM flavours with light $\nu$ oscillation data and $0\nu\beta\beta$\citep{Drewes:2016lqo,Hernandez:2016kel,Asaka:2016zib}\footnote{See also\citep{Bolton:2019pcu} for a discussion of the complementarity between $0\nu\beta\beta$ decays and colliders in the type I seesaw.} (if the sterile $\nu$ has a Majorana mass); see Fig.~\ref{fig:masterplot}. 
\item Finally, if HNL oscillations within the detector can be resolved, this can be used to indirectly constrain the HNL mass splitting\citep{Antusch:2017ebe,Antusch:2017pkq,Cvetic:2018elt,Cvetic:2019rms}, a parameter that strongly affects the BAU due to the resonant enhancement\citep{Dev:2017wwc,Garbrecht:2018mrp}, cf.~Fig.~\ref{leptogenesisn2}.
\end{itemize}
In addition, the HNLs can also be searched for using the meson decays, beta decays, electroweak precision data, and various cosmological and astrophysical observables; for a summary, see e.g.\citep{Bolton:2019pcu}. 

In the minimal realisation of the low scale seesaw, which phenomenologically also descibes the $\nu$MSM\citep{Asaka:2005an,Asaka:2005pn}, the parameter space is sufficiently constrained to fully test the model (in the sense of constraining all parameters in the Lagrangian) by combining all of these observables\citep{Hernandez:2016kel,Drewes:2016jae}.
Studies in a broader class of models will help to assess the potential of different experiments to discover the HNLs and, if they are found, probe the hypothesis that they are responsible for the origins of $\nu$ masses and the BAU.



%A  review volume dedicated to leptogenesis can be found, chapter by chapter,at\citep{Dev:2017trv,Drewes:2017zyw,Dev:2017wwc,Biondini:2017rpb,Chun:2017spz,Hagedorn:2017wjy}. 
%[[other Snowmass whitepaper (by Brian Shuve et al). ]]

% Computational Techniques: 
%     \begin{itemize}
%     \item Semi-classical Boltzmann
%     \item Flavor effects
%     \item CTP
% \end{itemize}
%Not to say much. Just link to recent reviews 
%(computational\citep{Garbrecht:2018mrp,Biondini:2017rpb}, IJMP review volume
%\citep{Dev:2017trv,Drewes:2017zyw,Dev:2017wwc,Biondini:2017rpb,Chun:2017spz,Hagedorn:2017wjy}) and other Snowmass whitepaper (by Brian Shuve et al). 



%\subsubsection{Parameter Space--\color{red}{Marco}}
%Money Plots by Marco for 2-HNL and 3-HNL cases (with some choice of $m_{\rm lightest}$ and initial condition for HNL)

\begin{figure*}
%\centering
 \begin{center}
\includegraphics[width=0.5\textwidth]{figures/n23snowmassV4.pdf}
\includegraphics[width=0.45\textwidth]{LNVvsLNC.pdf}
\caption
{
%\label{HNLsummary}
\emph{Left panel:}
%\emph{Bold green line:} Sensitivity of displaced vertex searches at FCC-ee with $5\times 10^{12}$ $Z$ bosons, assuming no background and $75\%$ reconstructed HNL decays with a displacement between $400\mu m$ and $1.22$m. For comparison, we show what CepC can achieve  with  $4.2\times 10^{12}$ $Z$ bosons for the same parameters.
%\emph{Bold turquoise line:} Gain in sensitivity if the maximal observable displacement is increased to $5$m with a HECATE-like detector\citep{Chrzaszcz:2020emg}.
Dark gray: Lower bound on the total HNL mixing from the requirement to explain the light $\nu$ oscillation data\citep{Esteban:2020cvm}.
Medium gray: Constraints on the active-sterile mixing $U_{\mu i}^2=\sum_\alpha|\theta_{\alpha i}|^2$ of HNLs from past experiments\citep{CHARM:1985nku,Abela:1981nf,Yamazaki:1984sj,E949:2014gsn,Bernardi:1987ek,NuTeV:1999kej,Vaitaitis:2000vc,CMS:2018iaf,DELPHI:1996qcc,ATLAS:2019kpx,CMS:2022fut}, obtained under the assumption that the HNLs exclusively mix with the second SM generation. %$U_{\alpha i}^2=\delta_{\alpha \mu}U^2$.
\emph{Light gray:} Lower bound on $U_\mu^2$ from BBN\citep{Sabti:2020yrt,Boyarsky:2020dzc}. Hashed orange and violet lines: Regions in which the observed baryon asymmetry of the universe can be explained with two\citep{Klaric:2020phc,Klaric:2021cpi} or three\citep{Drewes:2021nqr} HNL flavours and different initial conditions, as explained in the legend.
Other colourful lines: Estimated sensitivities of the LHC main detectors (taken from\citep{Izaguirre:2015pga,Drewes:2019fou,Pascoli:2018heg}) and NA62\citep{Drewes:2018gkc} as well as the sensitivities of selected planned or proposed experiments (DUNE\citep{Ballett:2019bgd},FASER2\citep{FASER:2018eoc},		 SHiP\citep{SHiP:2018xqw,Gorbunov:2020rjx}, MATHUSLA\citep{Curtin:2018mvb}, Codex-b\citep{Aielli:2019ivi}) as well as FCC-ee/CEPC\citep{Verhaaren:2022ify}, ILC and FCC-hh\citep{Antusch:2016ejd}.
%\color{red}
%Marco: This is a placeholder, to be replaced
%\color{black}
%Left: 
%Parameter range in which leptogenesis with three $\nu_R$ is possible\citep{Drewes:2021nqr} (between the black lines), compared to the  
%region ruled out in the global scan\citep{Chrzaszcz:2019inj} (The upper bound is dominated by the direct searches\citep{Shrock:1980vy,Abreu:1996pa,Bryman:2019bjg,NA62:2017qcd,NA62:2020mcv,Artamonov:2014urb,Bergsma:1985is,Bernardi:1987ek,Ruchayskiy:2011aa,Sirunyan:2018mtv,Aad:2019kiz,Sirunyan:2018xiv,Antusch:2017hhu,Shuve:2016muy,Vaitaitis:1999wq})
%complemented by the updated BBN bounds from\citep{Sabti:2020yrt,Boyarsky:2020dzc}
%(gray area) and the estimated sensitivities of the LHC main detectors (taken from\citep{Izaguirre:2015pga,Drewes:2019fou,Pascoli:2018heg}) and 
%		NA62\citep{Drewes:2018gkc} as well as the sensitivities of selected planned or proposed experiments (DUNE\citep{Ballett:2019bgd},
%			FASER2\citep{Ariga:2018uku},
%			SHiP\citep{Alekhin:2015byh,SHiP:2018xqw,Gorbunov:2020rjx}
%			MATHUSLA\citep{Curtin:2018mvb},
%		Codex-b\citep{Aielli:2019ivi}) as well as
%		future lepton colliders\citep{Antusch:2017pkq} or proton colliders\citep{Antusch:2016ejd}.
%Existing bounds\citep{Abreu:1996pa,NA62:2020mcv,Artamonov:2014urb,Bergsma:1985is,Bernardi:1987ek,Ruchayskiy:2011aa,Sirunyan:2018mtv,Aad:2019kiz,Sirunyan:2018xiv,Antusch:2017hhu,Shuve:2016muy,Vaitaitis:1999wq} %Aguilar-Arevalo:2017vlf,
%and sensitivity of selected proposed experimental searches (taken from\citep{Antusch:2016ejd,Beacham:2019nyx,Drewes:2019fou,Drewes:2018gkc,Izaguirre:2015pga,Pascoli:2018heg,Ballett:2019bgd}) for $N_i$ in the type I seesaw model.
\emph{Right panel:} Regions of mass- and mixing where $L$-violating processes are expected to be observable in the minimal type I seesaw model\citep{Drewes:2019byd}, quantified by the ratio $R_{ll}$ of $L$-violating to $L$-conserving HNL decays\citep{Anamiati:2016uxp}.
}\label{HNLsummary}
\end{center}
\end{figure*}




%\subsubsection{Theoretical Framework --\color{red}{Jacopo}}
%\subsubsection{Complementarity between frontiers--\color{red}{Bhupal,Julia,Shrock}}

%\begin{itemize}
%    \item Accelerator-based (beam-dump, collider)
%    \item Non accelerator-based (meson decays, $0\nu\beta\beta$, LFV)
    
    
%    \item Cosmological bounds (BBN, CMB, X-ray,...)
%\end{itemize}

%Some discussion on why $0\nu\beta\beta$ and lepton flavor violation are difficult to show in the summary plot. 



\section{Probing leptogenesis with TeV-scale lepton-number violation}\label{sec:HighScaleLepto} 
The testability and complementarity of different experimental frontiers make low-scale scale leptogenesis an interesting scenario. However, leptogenesis could be similarly realised via a high-scale leptogenesis mechanism, for instance the out-of-equilibrium decay of right-handed neutrinos (RHNs) featuring CP-violating interactions. However, as the expected RHN masses\citep{Davidson:2002qv} are typically beyond the reach of current and future colliders (with the exception of e.g. resonant leptogenesis\citep{Pilaftsis:2003gt}), these scenarios are usually difficult to probe. In order to ultimately experimentally pinpoint the mechanism behind the baryon asymmetry, alternative approaches have to be identified in order to also probe models at high scales. One powerful possibility is to instead "falsify" high-scale leptogenesis models via the observation of lepton-number violation around the TeV-scale.

For instance, the observation of a same-sign dilepton signature without missing energy at the LHC, would imply such a strong washout that an asymmetry generated at a higher scale would be directly washed out, ruling out the possibility to have generated the baryon asymmetry via high-scale leptogenesis models\citep{Deppisch:2013jxa}. For leptogenesis scenarios around the TeV-scale, such as resonant leptogenesis, an observation of such a signal would imply a lower limit on the CP asymmetry.

Another lepton-number violating observable is $0\nu\beta\beta$ decay. If a new physics mechanism of $0\nu\beta\beta$ decay other than the standard light $\nu$-exchange via the Weinberg operator is observed, typical scenarios of high-scale leptogenesis will be excluded unless the baryon asymmetry is protected via some new mechanism\citep{Deppisch:2015yqa,Deppisch:2017ecm}. Hence, once $0\nu\beta\beta$ decay is observed, the identification of its underlying mechanism will be of great importance. In order to confirm washout in all flavour sectors, an observation in all flavours or an additional measurement of lepton-flavour violation is required.

The interplay between collider probes and $0\nu\beta\beta$ decay is particularly important. Depending on the hierarchy of the new UV physics involved, one or the other probe can have the larger experimental reach\citep{Harz:2021psp}. While $0\nu\beta\beta$ decay is limited to the first generation only, collider searches allow also for same-sign signatures in second or third generation leptons. A detailed analysis\citep{Harz:2021psp} of a simplified model based on a dim-9 effective LNV interaction confirmed that an observation of lepton-number violation at current or future colliders or at $0\nu\beta\beta$ decay experiments would render single-flavour standard high-scale leptogenesis invalid. Again, for a conclusive exclusion, equilibration in all flavours has to be assured.

It is important to emphasize that these far-reaching consequences are not limited to high-scale leptogenesis scenarios, but similarly to other high-scale $\Delta(B-L) \neq 0$ baryogenesis scenarios due to the equilibration via the $(B+L)$-violating sphaleron processes. 
However, certain models that generate an asymmetry in a secluded dark sector or hide an asymmetry in a specific flavour might be exempt from such conclusions\citep{AristizabalSierra:2013lyx,Frandsen:2018jfi}.

In summary, experimental searches for lepton-number-violating signatures are highly relevant for probing high-scale leptogenesis and baryogenesis scenarios, even though the physics that generates the asymmetry might not be directly accessible. Hence, the observation of lepton-number violation at $0\nu\beta\beta$ decay experiments via a nonstandard mechanism or at current and future colliders, might point us to low-scale baryogenesis. Therefore, searches for lepton-number violation should be pursued with high priority at all frontiers.

